Robust Fusion Controller: Degradation-aware Image Fusion with Fine-grained Language Instructions

Current image fusion methods struggle to adapt to real-world environments encompassing diverse degradations with spatially varying characteristics. To address this challenge, we propose a robust fusion controller (RFC) capable of achieving degradation-aware image fusion through fine-grained language instructions, ensuring its reliable application in adverse environments. Specifically, RFC first parses language instructions to innovatively derive the functional condition and the spatial condition, where the former specifies the degradation type to remove, while the latter defines its spatial coverage. Then, a composite control priori is generated through a multi-condition coupling network, achieving a seamless transition from abstract language instructions to latent control variables. Subsequently, we design a hybrid attention-based fusion network to aggregate multi-modal information, in which the obtained composite control priori is deeply embedded to linearly modulate the intermediate fused features. To ensure the alignment between language instructions and control outcomes, we introduce a novel language-feature alignment loss, which constrains the consistency between feature-level gains and the composite control priori. Extensive experiments on publicly available datasets demonstrate that our RFC is robust against various composite degradations, particularly in highly challenging flare scenarios.

==> sec/2_formatting.tex <==
\section{Related Work}
\label{sec:related work}

\subsection{Vision-Language Model}
The transformer architecture introduced the self-attention mechanism, which successfully addressed the key performance and efficiency issues of traditional $\text{RNN}$ and $\text{LSTM}$ networks, significantly improving language modeling. This groundbreaking innovation has driven rapid development in the field of natural language processing, particularly facilitating the success of pre-trained models like BERT. The advent of Vision Transformer (ViT) brought the transformer architecture into the field of computer vision. It eliminated the reliance on traditional convolutional neural networks (CNNs), directly dividing images into patches and inputting them into a pure transformer, thereby achieving superior performance in image classification tasks compared to CNNs. These successful practices have driven the widespread application of transformer in multimodal learning. One notable example is CLIP, which explores the relationship between text and image and constructs a shared text-image embedding space. By leveraging contrastive learning on a large-scale text-image dataset, it achieves exceptional performance across a variety of cross-modal tasks, without the need for task-specific retraining. The success of CLIP has spawned many large models that combine 
\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{./Image/Net.png} 
	\caption{The overall framework of our proposed LREF.} 
	\label{net}
\end{figure*}
language with image processing. Among them, StyleCLIP extends a text-based image editing interface for StyleGAN that requires no manual effort, combining StyleGAN's powerful generative capabilities with CLIP's extraordinary visual concept understanding, enabling a variety of unique image operations. BLIP improves on CLIP and further enhances the joint representation between images and text through a self-supervised generative pre-training method, demonstrating superior performance in visual reasoning tasks. CLIPSeg, by extending a Transformer-based decoding network after the CLIP model, leverages CLIP’s powerful text-image alignment capabilities to successfully achieve zero-shot image segmentation.

\subsection{Fusion with Language}
With the rapid development of vision-language models, image fusion models incorporating language have gradually emerged. FILM was the first to integrate text guidance into image fusion algorithms, enhancing the fusion process by utilizing large language models to provide explicit texture descriptions of source images. This approach has achieved remarkable results in scenarios such as infrared-visible, medical, multi-exposure and multi-focus. TextFusion introduces semantic information about regions of interest into the image fusion process and creates a text-based image quality assessment method, enabling adaptive adjustments to the fusion results. Additionally, models such as FTP and LDL integrates high-level semantic descriptions from text to fuse the semantic information of infrared and visible images. Among these models, TeRF and Text-IF are closely related to our method. TeRF combines multiple large models to construct a text-guided, region-aware image fusion framework that enhances the regional information of the fused image based on text prompts, offering high interactivity and flexibility. Text-IF introduces a language interaction guidance module to fuse text and image information, successfully addressing the combined challenges of image fusion and degradation-aware processing.


